Multi-objective Generative Design of Three-Dimensional Composite Materials

Composite materials with 3D architectures are desirable in a variety of applications for the capability of tailoring their properties to meet multiple functional requirements. By the arrangement of materials' internal components, structure design is of great significance in tuning the properties of the composites. However, most of the composite structures are proposed by empirical designs following existing patterns. Hindered by the complexity of 3D structures, it is hard to extract customized structures with multiple desired properties from large design space. Here we report a multi-objective driven Wasserstein generative adversarial network (MDWGAN) to implement inverse designs of 3D composite structures according to given geometrical, structural and mechanical requirements. Our framework consists a GAN based network which generates 3D composite structures possessing with similar geometrical and structural features to the target dataset. Besides, multiple objectives are introduced to our framework for the control of mechanical property and isotropy of the composites. Real time calculation of the properties in training iterations is achieved by an accurate surrogate model. We constructed a small and concise dataset to illustrate our framework. With multiple objectives combined by their weight, and the 3D-GAN act as a soft constraint, our framework is proved to be capable of tuning the properties of the generated composites in multiple aspects, while keeping the selected features of different kinds of structures. The feasibility on small dataset and potential scalability on objectives of other properties make our work a novel, effective approach to provide fast, experience free composite structure designs for various functional materials.

==> mdwgan.tex <==
\section{Framework}\label{mdwgan}

We now present our key framework, Multi-objective Driven Wasserstein GAN (MDWGAN). Based on the the idea of Wasserstein GAN (WGAN)\cite{bib42_Arjovsky2017} and its modified version Wasserstein GAN (WGAN-GP) - Gradient Penalty\cite{bib44_Gulrajani2017}, we developed an extended 3D-WGAN-GP network to keep the structural similarity of generated structures and structures in the dataset. Furthermore, multiple objectives are combined with the original WGAN to control the properties of the composites. A surrogate model is introduced to calculate the properties in real time. Figure \ref{framework} gives an overview of our structure.

\begin{figure}[htbp]
\centering
\includegraphics[width=0.9\linewidth]{figures/Figure1_v2.jpg}
\caption{Schematic illustration of the framework for multi-objective generative design of 3D composite materials. {\bf{a}}. Overall framework. It is mainly a GAN based model whose generator and discriminator are build by 3D convolutional neural networks instead of 2D ones.  $\mathcal{O}_{sim}$ is the objective of generating similar structures with the dataset. A pre-trained surrogate model is introduced to predict the moduli of output composite structures from the generator. $\mathcal{O}_{lg}$ and $\mathcal{O}_{iso}$ are the objectives introduced to control the value and isotropy of the moduli, separately. {\bf{b}}. Voxel model of 20,000 stochastic and 20,000 center-symmetric composite structures are generated in a 6X6X6 space. The blue voxels represents for the reinforcements and the grey voxels represents for the matrix. The volume fraction \textit{$V_{f}$}=0.26, the Young's moduli and Poisson's ratio of the matrix and reinforcements {$E_{m}$}, {$E_{r}$}, {$\nu_{m}$} and {$\nu_{r}$}, are kept the same across all the structures. Single-axial compression simulations are performed to get the elastic response of the generated composite structures in \textit{x}, \textit{y} and \textit{z} direction. The dataset is constructed of structure tensors and moduli vectors \textit{$E_{xx}$}, {\it{$E_{yy}$}} and {\it{$E_{zz}$}} of the composite structures. {\bf{c}}. 3D Wasserstein GAN model for structure generation. 3D Transposed convolutions are used to generate new structures from random seed while 3D convolutions are used to discriminate the structures generated by traditional Wasserstein GAN loss $\mathcal{L}_{sim}^G$ and the moduli and isotropy objective losses $\mathcal{L}_{lg}$ and $\mathcal{L}_{iso}$ {\bf{d}}. Resnet-18 based surrogate models are used provide predicted moduli and isotropy for losses $\mathcal{L}_{lg}$ and $\mathcal{L}_{iso}$ calculation. The dataset construction by geometry generation and FEM simulations. }
\label{framework}
\end{figure} 

Basically, our main network has three key components: 3D-based generator, 3D-based discriminator and a pre-trained 3D surrogate model. 
%During the training process, there are two main training routes, one for 3D-based Generator and the other for 3D-based Discriminator. For the former training route, a random noise is produced and inputted to the 3D-based Generator. Then based on the random noise, the 3D-based Generator samples from a latent space. With the generated structure, the 3D-based Discriminator produces Loss $G_1$. Meanwhile, the generated structure is also sent to the pre-trained 3D Surrogate model. Based on the objectives we chose, we can calculate Loss $G_2$ or Loss $G_3$. Both Loss $G_1$ and Loss $G_2/G_3$ will be backpropogated to the 3D-based Generator. Note that in this procedure, the parameters of 3D-based Discriminator are frozen. For the latter training route, a random noise will be passed to the frozen 3D-based Generator and transformed into a structure. Also, we samples from the dataset and inputs both the generated fake structure and the real structure into the 3D-based Discriminator. Based on the output, we calculate Loss D and backpropogate it to the 3D-based Discriminator. 


\subsection{Multi-objective Driven 3D WGAN}\label{mdloss}

In our model, we mainly focus on three parts of objectives: $\mathcal{O}_{sim}$, $\mathcal{O}_{lg}$ and $\mathcal{O}_{iso}$. Each objectives gives a direction for the 3D-based generator to optimize and they are combined with different weights to achieve desired performances.

$\mathcal{O}_{sim}$ denotes the objective that imitates the data from the original training set. This objective can be also regarded as a soft constraint embedded in MDWGAN architecture. Since we aim at generating new structure designs, we does not intended to add hard constraints to limit the fraction of strong phase in the structure, the geometrical symmetry or the way of constituent material construction. Thus, we rely on a 3D, GAN-like network . That is, the 3D discriminator will restrain the behaviour of the 3D generator by distinguishing the structures produced by 3D-based generator from  the training data, based on their similarity. Note that this is a probabilistic prediction given by not only one parameter such as the fraction of strong phase, but also includes geometrical and structural features. 

$\mathcal{O}_{lg}$ describes the objective that the model has a tendency to generate structures with higher average moduli. Note that the tendency will not guarantee certainty on moduli optimization, but can increase the performance at an expectation degree. 

$\mathcal{O}_{iso}$ denotes the isometric moduli objective, which means that we encourage the 3D-based generator to generate structures with the same moduli in all three directions. Similar to $\mathcal{O}_{lg}$, it offers a tendency to the optimization of the 3D-based Generator model.

According to these objectives, we embodied those goals by the training losses. Those losses will gradually fine tune the 3D-based Generator model during the training process.

For objective $\mathcal{O}_{sim}$, we need to construct two parts of loss $\mathcal{L}_{sim}^D$ and $\mathcal{L}_{sim}^G$, which denotes the loss for 3D-based Discriminator and 3D-based Generator. We follows the discriminator loss $\mathcal{L}_{sim}^D$ from WGAN-GP\cite{bib44_Gulrajani2017} for our 3D-based discriminator, i.e.,
\begin{equation}\label{lossd}
    \mathcal{L}_{sim}^D=D_{w}(\Tilde{x})-D_{w}(x)+\lambda(\parallel\triangledown_{\Tilde{x}}D_{w}(x)\parallel_2-1)^2,
\end{equation}
where $D_w$ is the 3D-based discriminator, $\Tilde{x}$ is the fake sample generated by 3D-based generator $G$, $x$ is the real sample from our dataset, and $\lambda$ is the gradient panalty coefficient.

Again, we take the generator loss $\mathcal{L}_{sim}^G$ from WGAN-GP\cite{bib44_Gulrajani2017}, i.e., 
\begin{equation}\label{LG1}
    \mathcal{L}_{sim}^G=-D_{w}(\Tilde{x}),
\end{equation}

As mentioned in Figure \ref{framework}, we have designed multiple additional losses for different objectives. We construct the loss $\mathcal{L}_{lg}$ for objective $\mathcal{O}_{lg}$ as follows:
\begin{equation}\label{LG2}
    \mathcal{L}_{lg}=w_{lg}\cdot\frac{1}{B}\sum_{i=1}^B\parallel E_{goal}-S(\Tilde{x_i})\parallel^2_2,
\end{equation}
where $w_{lg}$ is a hyperparameter that denotes the weight of loss $\mathcal{L}_{lg}$, $B$ is the batch size, $E_{goal}$ is the modulus goal we set. $S$ is the pretrained surrogate model and $\Tilde{x_i}$ is the $i$-th sample in the batch. Thus, S($\Tilde{x_i}$) is the predicted modulus of generated sample.

Also, we construct the loss $\mathcal{L}_{iso}$ for isotropy objective $\mathcal{O}_{iso}$, which can be represented as follows:
\begin{equation}\label{LG3}
    \mathcal{L}_{iso}=w_{iso}\cdot\frac{1}{B}\sum_{i=1}^B\sum_{j,k\in\{X,Y,Z\},j\neq k} (S_j(\Tilde{x_i})-S_k(\Tilde{x_i}))^2,
\end{equation}
where $w_{iso}$ is a hyperparameter that denotes the weight of loss $\mathcal{L}_{iso}$ and $S_{X},S_{Y},S_{Z}$ denotes the calculated moduli of $X,Y,Z$ direction. 


\subsection{3D Surrogate Model}\label{surr}
As introduced previously, our MDWGAN model introduces a special component - 3D Surrogate Model (Fig \ref{framework}). Our 3D Surrogate Model is based on ResNet-18\cite{bib43_He2015}. Different from its original version, we switch its 2D convolutional networks to 3D convolutional networks and modify its pooling layers. We pre-trained the model before appending it to our framework (See method). Our pre-trained surrogate model can estimate the moduli of a given structure rapidly compared to FEM, which allows us to significantly reduce our training time.

\iffalse
\begin{figure}[htbp]
	%\addtocounter{figure}{-1} 
	\subfigure{
		\begin{minipage}[t]{0.305\linewidth}%%%%%%%%%note2
			\centering
			\includegraphics[width=0.99\linewidth]{figures/Surrogate_result_plot_1.png}
		\end{minipage}
	}
	\subfigure{
		\begin{minipage}[t]{0.305\linewidth}%%%%%%%%%note2
			\centering
			\includegraphics[width=0.99\linewidth]{figures/Surrogate_result_plot_2.png}
		\end{minipage}
	}
	\subfigure{
		\begin{minipage}[t]{0.305\linewidth}%%%%%%%%%note2
			\centering
			\includegraphics[width=0.99\linewidth]{figures/Surrogate_result_plot_3.png}
		\end{minipage}
	}
	\caption{Comparison between real moduli and moduli calculated by surrogate model on x, y and z axes.}
	\label{surrfig}
\end{figure}
\fi

\begin{figure}[htbp]
	\centering
	\includegraphics[width=0.99\linewidth]{figures/surr_fem_v3.jpg}
	\caption{Comparison between real moduli and moduli calculated by surrogate model on x, y and z axes.}
	\label{surrfig}
\end{figure}
Figure \ref{surrfig} gives us a view of calculated moduli versus real moduli. Based on our calculation, the variance of the real moduli is $3.63\times 10^{-2}$, while the mean square error (MSE) between the moduli from our surrogate model and the real moduli is $2.02\times 10^{-4}$.  This result enables us to use the pre-trained 3D surrogate model to approximate the moduli of generated instance and accelerate the training process.


